Role of coupled electrochemistry and stress on the Li-anode instability: A continuum approach

We present a coupled mechanistic approach that elucidates the intricate interplay between stress and electrochemistry, enabling the prediction of the onset of instabilities in Li-metal anodes and the solid electrolyte interphase (SEI) in liquid-electrolyte Li-metal batteries. Our continuum theory considers a two-way coupling between stress and electrochemistry, includes Li and electron transport through SEI, incorporates effects of Li viscoplasticity, includes SEI and electrolyte interface surface energy and evaluates crucial roles of these mechanistic effects on the continuously evolving anode surface due to the viscoplastic deformation of lithium. In the model, spatial current density evolves with the stress-induced potential across the deformed anode/SEI interface. We assume SEI as a homogeneous, artificial layer on the Li-anode, which allows the investigation of the mechanical and electrochemical properties of the SEI systematically. Subsequently, we solve a set of coupled electrochemistry and displacement equations within the SEI and anode domains. The model is implemented numerically by writing a user element subroutine in Abaqus/Standard. We conduct numerical simulations under various galvanostatic conditions and SEI properties and predict conditions for anode instability. We find that Li viscoplasticity is one of the key attributes that drives instability in the Li-anode and show that applying a soft artificial SEI layer on the Li-anode to minimize viscoplastic deformation can be an effective method. We also report the role of artificial SEI elasticity and thickness on anode stability. Selected stability maps are provided as a design aid for artificial SEI.

==> MACROS_BK4.tex <==
%%%%%%%%%%%%% MACROS

\newcommand{\calA}{\mathcal{A}}%
\newcommand{\calB}{\mathcal{B}}%
\newcommand{\calC}{\mathcal{C}}%
\newcommand{\calD}{\mathcal{D}}%
\newcommand{\calE}{\mathcal{E}}%
\newcommand{\calF}{\mathcal{F}}%
\newcommand{\calH}{\mathcal{H}}%
\newcommand{\calI}{\mathcal{I}}%
\newcommand{\calJ}{\mathcal{J}}%
\newcommand{\calK}{\mathcal{K}}%
\newcommand{\calL}{\mathcal{L}}%
\newcommand{\calM}{\mathcal{M}}%
\newcommand{\calN}{\mathcal{N}}%
\newcommand{\calP}{\mathcal{P}}%
\newcommand{\calQ}{\mathcal{Q}}%
\newcommand{\calR}{\mathcal{R}}%
\newcommand{\calS}{\mathcal{S}}%
\newcommand{\calV}{\mathcal{V}}%
\newcommand{\calW}{\mathcal{W}}%
\newcommand{\calX}{\mathcal{X}}%
\newcommand{\calT}{\mathcal{T}}%
%
%
\newcommand{\bfa}{{\bf a}}\newcommand{\bfA}{{\bf A}}%
\newcommand{\bfb}{{\bf b}}\newcommand{\bfB}{{\bf B}}%
\newcommand{\bfc}{{\bf c}}\newcommand{\bfC}{{\bf C}}%
\newcommand{\bfd}{{\bf d}}\newcommand{\bfD}{{\bf D}}%
\newcommand{\bfe}{{\bf e}}\newcommand{\bfE}{{\bf E}}%
\newcommand{\bff}{{\bf f}}\newcommand{\bfF}{{\bf F}}%
\newcommand{\bfg}{{\bf g}}\newcommand{\bfG}{{\bf G}}%
\newcommand{\bfh}{{\bf h}}\newcommand{\bfH}{{\bf H}}%
\newcommand{\bfi}{{\bf i}}\newcommand{\bfI}{{\bf I}}%
\newcommand{\bfj}{{\bf j}}\newcommand{\bfJ}{{\bf J}}%
\newcommand{\bfk}{{\bf k}}\newcommand{\bfK}{{\bf K}}%
\newcommand{\bfl}{{\bf l}}\newcommand{\bfL}{{\bf L}}%
\newcommand{\bfm}{{\bf m}}\newcommand{\bfM}{{\bf M}}%
\newcommand{\bfn}{{\bf n}}\newcommand{\bfN}{{\bf N}}%
\newcommand{\bfo}{{\bf o}}\newcommand{\bfO}{{\bf O}}%
\newcommand{\bfp}{{\bf p}}\newcommand{\bfP}{{\bf P}}%
\newcommand{\bfq}{{\bf q}}\newcommand{\bfQ}{{\bf Q}}%
\newcommand{\bfr}{{\bf r}}\newcommand{\bfR}{{\bf R}}%
\newcommand{\bfs}{{\bf s}}\newcommand{\bfS}{{\bf S}}%
\newcommand{\bft}{{\bf t}}\newcommand{\bfT}{{\bf T}}%
\newcommand{\bfu}{{\bf u}}\newcommand{\bfU}{{\bf U}}%
\newcommand{\bfv}{{\bf v}}\newcommand{\bfV}{{\bf V}}%
\newcommand{\bfw}{{\bf w}}\newcommand{\bfW}{{\bf W}}%
\newcommand{\bfx}{{\bf x}}\newcommand{\bfX}{{\bf X}}%
\newcommand{\bfy}{{\bf y}}\newcommand{\bfY}{{\bf Y}}%
\newcommand{\bfz}{{\bf z}}\newcommand{\bfZ}{{\bf Z}}%
\newcommand{\bfell}{\boldsymbol{\ell}}%
\newcommand{\bfimath}{\boldsymbol{\imath}}%
\newcommand{\bfjmath}{\boldsymbol{\jmath}}%
\newcommand{\bfwp}{\boldsymbol{\wp}}%
\newcommand{\bfalpha}{\boldsymbol{\alpha}}%
\newcommand{\bfbeta}{\boldsymbol{\beta}}%
\newcommand{\bfgamma}{\boldsymbol{\gamma}}%
\newcommand{\bfdelta}{\boldsymbol{\delta}}%
\newcommand{\bfepsilon}{\boldsymbol{\epsilon}}%
\newcommand{\bfzeta}{\boldsymbol{\zeta}}%
\newcommand{\bfeta}{\boldsymbol{\eta}}%
\newcommand{\bftheta}{\boldsymbol{\theta}}%
\newcommand{\bfiota}{\boldsymbol{\iota}}%
\newcommand{\bfkappa}{\boldsymbol{\kappa}}%
\newcommand{\bflambda}{\boldsymbol{\lambda}}%
\newcommand{\bfmu}{\boldsymbol{\mu}}%
\newcommand{\bfnu}{\boldsymbol{\nu}}%
\newcommand{\bfxi}{\boldsymbol{\xi}}%
\newcommand{\bfpi}{\boldsymbol{\pi}}%
\newcommand{\bfrho}{\boldsymbol{\rho}}%
\newcommand{\bfsigma}{\boldsymbol{\sigma}}%
\newcommand{\bftau}{\boldsymbol{\tau}}%
\newcommand{\bfupsilon}{\boldsymbol{\upsilon}}%
\newcommand{\bfphi}{\boldsymbol{\phi}}%
\newcommand{\bfchi}{\boldsymbol{\chi}}%
\newcommand{\bfpsi}{\boldsymbol{\psi}}%
\newcommand{\bfomega}{\boldsymbol{\omega}}%
\newcommand{\bfvarepsilon}{\boldsymbol{\varepsilon}}%
\newcommand{\bfvartheta}{\boldsymbol{\vartheta}}%
\newcommand{\bfvarpi}{\boldsymbol{\vaarphi}}%
\newcommand{\bfvarrho}{\boldsymbol{\varrho}}%
\newcommand{\bfvarsigma}{\boldsymbol{\varsigma}}%
\newcommand{\bfvarphi}{\boldsymbol{\varphi}}%
%
\newfont{\tenbfit}{cmmib10}%
\newfont{\svnbfit}{cmmib8}%
\newfont{\tenbfsl}{cmbxti10}% <-- for idem tensor
\newcommand{\bfGamma}{\mbox{\tenbfit\char'00\/}}%
\newcommand{\bfDelta}{\mbox{\tenbfit\char'01\/}}%
%\newcommand{\bfTheta}{\mbox{\tenbfit\char'02\/}}%
\newcommand{\bfTheta}{\boldsymbol{\Theta}}%
\newcommand{\bfLambda}{\boldsymbol{\Lambda}}%
\newcommand{\bfXi}{\mbox{\tenbfit\char'04\/}}%
\newcommand{\bfPi}{\mbox{\tenbfit\char'05\/}}%
\newcommand{\bfSigma}{\boldsymbol{\Sigma}}%
\newcommand{\bfUpsilon}{\mbox{\tenbfit\char'07\/}}%
\newcommand{\bfPhi}{\boldsymbol{\Phi}}
\newcommand{\bfPsi}{\mbox{\tenbfit\char'11\/}}%
\newcommand{\bfOmega}{\boldsymbol{\Omega}}
\newcommand{\sbfGamma}{\mbox{\svnbfit\char'00\/}}%
\newcommand{\sbfDelta}{\mbox{\svnbfit\char'01\/}}%
\newcommand{\sbfTheta}{\mbox{\svnbfit\char'02\/}}%
\newcommand{\sbfLambda}{\mbox{\svnbfit\char'03\/}}%
\newcommand{\sbfXi}{\mbox{\svnbfit\char'04\/}}%
\newcommand{\sbfPi}{\mbox{\svnbfit\char'05\/}}%
\newcommand{\sbfSigma}{\mbox{\svnbfit\char'06\/}}%
\newcommand{\sbfUpsilon}{\mbox{\svnbfit\char'07\/}}%
\newcommand{\sbfPhi}{\mbox{\svnbfit\char'10\/}}%
\newcommand{\sbfPsi}{\mbox{\svnbfit\char'11\/}}%
\newcommand{\sbfOmega}{\mbox{\svnbfit\char'12\/}}%
%
\newfont{\mmit}{cmmi10}% scaled 1200
\newfont{\smit}{cmmi9}%  scaled 1200
\newfont{\bfMit}{cmmi5}%  scaled 1200
%
\newcommand{\iGamma}{\mbox{\mmit\char'00\/}}%
\newcommand{\iDelta}{\mbox{\mmit\char'01\/}}%
\newcommand{\iTheta}{\mbox{\mmit\char'02\/}}%
\newcommand{\iLambda}{\mbox{\mmit\char'03\/}}%
\newcommand{\iXi}{\mbox{\mmit\char'04\/}}%
\newcommand{\iPi}{\mbox{\mmit\char'05\/}}%
\newcommand{\iSigma}{\mbox{\mmit\char'06\/}}%
\newcommand{\iUpsilon}{\mbox{\mmit\char'07\/}}%
\newcommand{\iPhi}{\mbox{\mmit\char'10\/}}%
\newcommand{\iPsi}{\mbox{\mmit\char'11\/}}%
\newcommand{\iOmega}{\mbox{\mmit\char'12\/}}%
%
\newcommand{\siGamma}{\mbox{\smit\char'00\/}}%
\newcommand{\siDelta}{\mbox{\smit\char'01\/}}%
\newcommand{\siTheta}{\mbox{\smit\char'02\/}}%
\newcommand{\siLambda}{\mbox{\smit\char'03\/}}%
\newcommand{\siXi}{\mbox{\smit\char'04\/}}%
\newcommand{\siPi}{\mbox{\smit\char'05\/}}%
\newcommand{\siSigma}{\mbox{\smit\char'06\/}}%
\newcommand{\siUpsilon}{\mbox{\smit\char'07\/}}%
\newcommand{\siPhi}{\mbox{\smit\char'10\/}}%
\newcommand{\siPsi}{\mbox{\smit\char'11\/}}%
\newcommand{\siOmega}{\mbox{\smit\char'12\/}}%
%
\newcommand{\ssiGamma}{\mbox{\bfMit\char'00\/}}%
\newcommand{\ssiDelta}{\mbox{\bfMit\char'01\/}}%
\newcommand{\ssiTheta}{\mbox{\bfMit\char'02\/}}%
\newcommand{\ssiLambda}{\mbox{\bfMit\char'03\/}}%
\newcommand{\ssiXi}{\mbox{\bfMit\char'04\/}}%
\newcommand{\ssiPi}{\mbox{\bfMit\char'05\/}}%
\newcommand{\ssiSigma}{\mbox{\bfMit\char'06\/}}%
\newcommand{\ssiUpsilon}{\mbox{\bfMit\char'07\/}}%
\newcommand{\ssiPhi}{\mbox{\bfMit\char'10\/}}%
\newcommand{\ssiPsi}{\mbox{\bfMit\char'11\/}}%
\newcommand{\ssiOmega}{\mbox{\bfMit\char'12\/}}%
%
\newfont{\tenbbb}{msbm10}%
\newfont{\svnbbb}{msbm8}%
%
\newcommand{\bbA}{\mbox{\tenbbb A\/}}%
\newcommand{\bbB}{\mbox{\tenbbb B\/}}%
\newcommand{\bbC}{\mbox{\tenbbb C\/}}%
\newcommand{\bbD}{\mbox{\tenbbb D\/}}%
\newcommand{\bbE}{\mbox{\tenbbb E\/}}%
\newcommand{\bbF}{\mbox{\tenbbb F\/}}%
\newcommand{\bbG}{\mbox{\tenbbb G\/}}%
\newcommand{\bbH}{\mbox{\tenbbb H\/}}%
\newcommand{\bbI}{\mbox{\tenbbb I\/}}%
\newcommand{\bbJ}{\mbox{\tenbbb J\/}}%
\newcommand{\bbK}{\mbox{\tenbbb K\/}}%
\newcommand{\bbL}{\mbox{\tenbbb L\/}}%
\newcommand{\bbM}{\mbox{\tenbbb M\/}}%
\newcommand{\bbN}{\mbox{\tenbbb N\/}}%
\newcommand{\bbO}{\mbox{\tenbbb O\/}}%
\newcommand{\bbP}{\mbox{\tenbbb P\/}}%
\newcommand{\bbQ}{\mbox{\tenbbb Q\/}}%
\newcommand{\bbR}{\mbox{\tenbbb R\/}}%
\newcommand{\bbS}{\mbox{\tenbbb S\/}}%
\newcommand{\bbT}{\mbox{\tenbbb T\/}}%
\newcommand{\bbU}{\mbox{\tenbbb U\/}}%
\newcommand{\bbV}{\mbox{\tenbbb V\/}}%
\newcommand{\bbW}{\mbox{\tenbbb W\/}}%
\newcommand{\bbX}{\mbox{\tenbbb X\/}}%
\newcommand{\bbY}{\mbox{\tenbbb Y\/}}%
\newcommand{\bbZ}{\mbox{\tenbbb Z\/}}%
%
\newcommand{\sbbA}{\mbox{\svnbbb A\/}}%
\newcommand{\sbbB}{\mbox{\svnbbb B\/}}%
\newcommand{\sbbC}{\mbox{\svnbbb C\/}}%
\newcommand{\sbbD}{\mbox{\svnbbb D\/}}%
\newcommand{\sbbE}{\mbox{\svnbbb E\/}}%
\newcommand{\sbbF}{\mbox{\svnbbb F\/}}%
\newcommand{\sbbG}{\mbox{\svnbbb G\/}}%
\newcommand{\sbbH}{\mbox{\svnbbb H\/}}%
\newcommand{\sbbI}{\mbox{\svnbbb I\/}}%
\newcommand{\sbbJ}{\mbox{\svnbbb J\/}}%
\newcommand{\sbbK}{\mbox{\svnbbb K\/}}%
\newcommand{\sbbL}{\mbox{\svnbbb L\/}}%
\newcommand{\sbbM}{\mbox{\svnbbb M\/}}%
\newcommand{\sbbN}{\mbox{\svnbbb N\/}}%
\newcommand{\sbbO}{\mbox{\svnbbb O\/}}%
\newcommand{\sbbP}{\mbox{\svnbbb P\/}}%
\newcommand{\sbbQ}{\mbox{\svnbbb Q\/}}%
\newcommand{\sbbR}{\mbox{\svnbbb R\/}}%
\newcommand{\sbbS}{\mbox{\svnbbb S\/}}%
\newcommand{\sbbT}{\mbox{\svnbbb T\/}}%
\newcommand{\sbbU}{\mbox{\svnbbb U\/}}%
\newcommand{\sbbV}{\mbox{\svnbbb V\/}}%
\newcommand{\sbbW}{\mbox{\svnbbb W\/}}%
\newcommand{\sbbX}{\mbox{\svnbbb X\/}}%
\newcommand{\sbbY}{\mbox{\svnbbb Y\/}}%
\newcommand{\sbbZ}{\mbox{\svnbbb Z\/}}%
%
\newfont{\tenssit}{cmssqi8 at 10pt}%
\newfont{\svnssit}{cmssqi8 at 7pt}%
%
\newcommand{\ssa}{\mbox{\tenssit a\/}}%
\newcommand{\ssA}{\mbox{\tenssit A\/}}%
\newcommand{\ssb}{\mbox{\tenssit b\/}}%
\newcommand{\ssB}{\mbox{\tenssit B\/}}%
\newcommand{\ssc}{\mbox{\tenssit c\/}}%
\newcommand{\ssC}{\mbox{\tenssit C\/}}%
\newcommand{\ssd}{\mbox{\tenssit d\/}}%
\newcommand{\ssD}{\mbox{\tenssit D\/}}%
\newcommand{\sse}{\mbox{\tenssit e\/}}%
\newcommand{\ssE}{\mbox{\tenssit E\/}}%
\newcommand{\ssf}{\mbox{\tenssit f\/}}%
\newcommand{\ssF}{\mbox{\tenssit F\/}}%
\newcommand{\ssg}{\mbox{\tenssit g\/}}%
\newcommand{\ssG}{\mbox{\tenssit G\/}}%
\newcommand{\ssh}{\mbox{\tenssit h\/}}%
\newcommand{\ssH}{\mbox{\tenssit H\/}}%
\newcommand{\ssi}{\mbox{\tenssit i\/}}%
\newcommand{\ssI}{\mbox{\tenssit I\/}}%
\newcommand{\ssj}{\mbox{\tenssit j\/}}%
\newcommand{\ssJ}{\mbox{\tenssit J\/}}%
\newcommand{\ssk}{\mbox{\tenssit k\/}}%
\newcommand{\ssK}{\mbox{\tenssit K\/}}%
\newcommand{\ssl}{\mbox{\tenssit l\/}}%
\newcommand{\ssL}{\mbox{\tenssit L\/}}%
\newcommand{\ssm}{\mbox{\tenssit m\/}}%
\newcommand{\ssM}{\mbox{\tenssit M\/}}%
\newcommand{\ssn}{\mbox{\tenssit n\/}}%
\newcommand{\ssN}{\mbox{\tenssit N\/}}%
\newcommand{\sso}{\mbox{\tenssit o\/}}%
\newcommand{\ssO}{\mbox{\tenssit O\/}}%
\newcommand{\ssp}{\mbox{\tenssit p\/}}%
\newcommand{\ssP}{\mbox{\tenssit P\/}}%
\newcommand{\ssq}{\mbox{\tenssit q\/}}%
\newcommand{\ssQ}{\mbox{\tenssit Q\/}}%
\newcommand{\ssr}{\mbox{\tenssit r\/}}%
\newcommand{\ssR}{\mbox{\tenssit R\/}}%
\newcommand{\sss}{\mbox{\tenssit s\/}}%
\newcommand{\ssS}{\mbox{\tenssit S\/}}%
\newcommand{\sst}{\mbox{\tenssit t\/}}%
\newcommand{\ssT}{\mbox{\tenssit T\/}}%
\newcommand{\ssu}{\mbox{\tenssit u\/}}%
\newcommand{\ssU}{\mbox{\tenssit U\/}}%
\newcommand{\ssv}{\mbox{\tenssit v\/}}%
\newcommand{\ssV}{\mbox{\tenssit V\/}}%
\newcommand{\ssw}{\mbox{\tenssit w\/}}%
\newcommand{\ssW}{\mbox{\tenssit W\/}}%
\newcommand{\ssx}{\mbox{\tenssit x\/}}%
\newcommand{\ssX}{\mbox{\tenssit X\/}}%
\newcommand{\ssy}{\mbox{\tenssit y\/}}%
\newcommand{\ssY}{\mbox{\tenssit Y\/}}%
\newcommand{\ssz}{\mbox{\tenssit z\/}}%
\newcommand{\ssZ}{\mbox{\tenssit Z\/}}%
%
\newcommand{\sssa}{\mbox{\svnssit a\/}}%
\newcommand{\sssA}{\mbox{\svnssit A\/}}%
\newcommand{\sssb}{\mbox{\svnssit b\/}}%
\newcommand{\sssB}{\mbox{\svnssit B\/}}%
\newcommand{\sssc}{\mbox{\svnssit c\/}}%
\newcommand{\sssC}{\mbox{\svnssit C\/}}%
\newcommand{\sssd}{\mbox{\svnssit d\/}}%
\newcommand{\sssD}{\mbox{\svnssit D\/}}%
\newcommand{\ssse}{\mbox{\svnssit e\/}}%
\newcommand{\sssE}{\mbox{\svnssit E\/}}%
\newcommand{\sssf}{\mbox{\svnssit f\/}}%
\newcommand{\sssF}{\mbox{\svnssit F\/}}%
\newcommand{\sssg}{\mbox{\svnssit g\/}}%
\newcommand{\sssG}{\mbox{\svnssit G\/}}%
\newcommand{\sssh}{\mbox{\svnssit h\/}}%
\newcommand{\sssH}{\mbox{\svnssit H\/}}%
\newcommand{\sssi}{\mbox{\svnssit i\/}}%
\newcommand{\sssI}{\mbox{\svnssit I\/}}%
\newcommand{\sssj}{\mbox{\svnssit j\/}}%
\newcommand{\sssJ}{\mbox{\svnssit J\/}}%
\newcommand{\sssk}{\mbox{\svnssit k\/}}%
\newcommand{\sssK}{\mbox{\svnssit K\/}}%
\newcommand{\sssl}{\mbox{\svnssit l\/}}%
\newcommand{\sssL}{\mbox{\svnssit L\/}}%
\newcommand{\sssm}{\mbox{\svnssit m\/}}%
\newcommand{\sssM}{\mbox{\svnssit M\/}}%
\newcommand{\sssn}{\mbox{\svnssit n\/}}%
\newcommand{\sssN}{\mbox{\svnssit N\/}}%
\newcommand{\ssso}{\mbox{\svnssit o\/}}%
\newcommand{\sssO}{\mbox{\svnssit O\/}}%
\newcommand{\sssp}{\mbox{\svnssit p\/}}%
\newcommand{\sssP}{\mbox{\svnssit P\/}}%
\newcommand{\sssq}{\mbox{\svnssit q\/}}%
\newcommand{\sssQ}{\mbox{\svnssit Q\/}}%
\newcommand{\sssr}{\mbox{\svnssit r\/}}%
\newcommand{\sssR}{\mbox{\svnssit R\/}}%
\newcommand{\ssss}{\mbox{\svnssit s\/}}%
\newcommand{\sssS}{\mbox{\svnssit S\/}}%
\newcommand{\ssst}{\mbox{\svnssit t\/}}%
\newcommand{\sssT}{\mbox{\svnssit T\/}}%
\newcommand{\sssu}{\mbox{\svnssit u\/}}%
\newcommand{\sssU}{\mbox{\svnssit U\/}}%
\newcommand{\sssv}{\mbox{\svnssit v\/}}%
\newcommand{\sssV}{\mbox{\svnssit V\/}}%
\newcommand{\sssw}{\mbox{\svnssit w\/}}%
\newcommand{\sssW}{\mbox{\svnssit W\/}}%
\newcommand{\sssx}{\mbox{\svnssit x\/}}%
\newcommand{\sssX}{\mbox{\svnssit X\/}}%
\newcommand{\sssy}{\mbox{\svnssit y\/}}%
\newcommand{\sssY}{\mbox{\svnssit Y\/}}%
\newcommand{\sssz}{\mbox{\svnssit z\/}}%
\newcommand{\sssZ}{\mbox{\svnssit Z\/}}%
%
%
\newfont{\gothic}{eufm10}%
\newfont{\sgothic}{eufm7}%
%
\newcommand{\gta}{\mbox{\gothic a\/}}%
\newcommand{\gtA}{\mbox{\gothic A\/}}%
\newcommand{\gtb}{\mbox{\gothic b\/}}%
\newcommand{\gtB}{\mbox{\gothic B\/}}%
\newcommand{\gtc}{\mbox{\gothic c\/}}%
\newcommand{\gtC}{\mbox{\gothic C\/}}%
\newcommand{\gtd}{\mbox{\gothic d\/}}%
\newcommand{\gtD}{\mbox{\gothic D\/}}%
\newcommand{\gte}{\mbox{\gothic e\/}}%
\newcommand{\gtE}{\mbox{\gothic E\/}}%
\newcommand{\gtf}{\mbox{\gothic f\/}}%
\newcommand{\gtF}{\mbox{\gothic F\/}}%
\newcommand{\gtg}{\mbox{\gothic g\/}}%
\newcommand{\gtG}{\mbox{\gothic G\/}}%
\newcommand{\gth}{\mbox{\gothic h\/}}%
\newcommand{\gtH}{\mbox{\gothic H\/}}%
\newcommand{\gti}{\mbox{\gothic i\/}}%
\newcommand{\gtI}{\mbox{\gothic I\/}}%
\newcommand{\gtj}{\mbox{\gothic j\/}}%
\newcommand{\gtJ}{\mbox{\gothic J\/}}%
\newcommand{\gtk}{\mbox{\gothic k\/}}%
\newcommand{\gtK}{\mbox{\gothic K\/}}%
\newcommand{\gtl}{\mbox{\gothic l\/}}%
\newcommand{\gtL}{\mbox{\gothic L\/}}%
\newcommand{\gtm}{\mbox{\gothic m\/}}%
\newcommand{\gtM}{\mbox{\gothic M\/}}%
\newcommand{\gtn}{\mbox{\gothic n\/}}%
\newcommand{\gtN}{\mbox{\gothic N\/}}%
\newcommand{\gto}{\mbox{\gothic o\/}}%
\newcommand{\gtO}{\mbox{\gothic O\/}}%
\newcommand{\gtp}{\mbox{\gothic p\/}}%
\newcommand{\gtP}{\mbox{\gothic P\/}}%
\newcommand{\gtq}{\mbox{\gothic q\/}}%
\newcommand{\gtQ}{\mbox{\gothic Q\/}}%
\newcommand{\gtr}{\mbox{\gothic r\/}}%
\newcommand{\gtR}{\mbox{\gothic R\/}}%
\newcommand{\gts}{\mbox{\gothic s\/}}%
\newcommand{\gtS}{\mbox{\gothic S\/}}%
\newcommand{\gtt}{\mbox{\gothic t\/}}%
\newcommand{\gtT}{\mbox{\gothic T\/}}%
\newcommand{\gtu}{\mbox{\gothic u\/}}%
\newcommand{\gtU}{\mbox{\gothic U\/}}%
\newcommand{\gtv}{\mbox{\gothic v\/}}%
\newcommand{\gtV}{\mbox{\gothic V\/}}%
\newcommand{\gtw}{\mbox{\gothic w\/}}%
\newcommand{\gtW}{\mbox{\gothic W\/}}%
\newcommand{\gtx}{\mbox{\gothic x\/}}%
\newcommand{\gtX}{\mbox{\gothic X\/}}%
\newcommand{\gty}{\mbox{\gothic y\/}}%
\newcommand{\gtY}{\mbox{\gothic Y\/}}%
\newcommand{\gtz}{\mbox{\gothic z\/}}%
\newcommand{\gtZ}{\mbox{\gothic Z\/}}%
\newcommand{\sgta}{\mbox{\sgothic a\/}}%
\newcommand{\sgtA}{\mbox{\sgothic A\/}}%
\newcommand{\sgtb}{\mbox{\sgothic b\/}}%
\newcommand{\sgtB}{\mbox{\sgothic B\/}}%
\newcommand{\sgtc}{\mbox{\sgothic c\/}}%
\newcommand{\sgtC}{\mbox{\sgothic C\/}}%
\newcommand{\sgtd}{\mbox{\sgothic d\/}}%
\newcommand{\sgtD}{\mbox{\sgothic D\/}}%
\newcommand{\sgte}{\mbox{\sgothic e\/}}%
\newcommand{\sgtE}{\mbox{\sgothic E\/}}%
\newcommand{\sgtf}{\mbox{\sgothic f\/}}%
\newcommand{\sgtF}{\mbox{\sgothic F\/}}%
\newcommand{\sgtg}{\mbox{\sgothic g\/}}%
\newcommand{\sgtG}{\mbox{\sgothic G\/}}%
\newcommand{\sgth}{\mbox{\sgothic h\/}}%
\newcommand{\sgtH}{\mbox{\sgothic H\/}}%
\newcommand{\sgti}{\mbox{\sgothic i\/}}%
\newcommand{\sgtI}{\mbox{\sgothic I\/}}%
\newcommand{\sgtj}{\mbox{\sgothic j\/}}%
\newcommand{\sgtJ}{\mbox{\sgothic J\/}}%
\newcommand{\sgtk}{\mbox{\sgothic k\/}}%
\newcommand{\sgtK}{\mbox{\sgothic K\/}}%
\newcommand{\sgtl}{\mbox{\sgothic l\/}}%
\newcommand{\sgtL}{\mbox{\sgothic L\/}}%
\newcommand{\sgtm}{\mbox{\sgothic m\/}}%
\newcommand{\sgtM}{\mbox{\sgothic M\/}}%
\newcommand{\sgtn}{\mbox{\sgothic n\/}}%
\newcommand{\sgtN}{\mbox{\sgothic N\/}}%
\newcommand{\sgto}{\mbox{\sgothic o\/}}%
\newcommand{\sgtO}{\mbox{\sgothic O\/}}%
\newcommand{\sgtp}{\mbox{\sgothic p\/}}%
\newcommand{\sgtP}{\mbox{\sgothic P\/}}%
\newcommand{\sgtq}{\mbox{\sgothic q\/}}%
\newcommand{\sgtQ}{\mbox{\sgothic Q\/}}%
\newcommand{\sgtr}{\mbox{\sgothic r\/}}%
\newcommand{\sgtR}{\mbox{\sgothic R\/}}%
\newcommand{\sgts}{\mbox{\sgothic s\/}}%
\newcommand{\sgtS}{\mbox{\sgothic S\/}}%
\newcommand{\sgtt}{\mbox{\sgothic t\/}}%
\newcommand{\sgtT}{\mbox{\sgothic T\/}}%
\newcommand{\sgtu}{\mbox{\sgothic u\/}}%
\newcommand{\sgtU}{\mbox{\sgothic U\/}}%
\newcommand{\sgtv}{\mbox{\sgothic v\/}}%
\newcommand{\sgtV}{\mbox{\sgothic V\/}}%
\newcommand{\sgtw}{\mbox{\sgothic w\/}}%
\newcommand{\sgtW}{\mbox{\sgothic W\/}}%
\newcommand{\sgtx}{\mbox{\sgothic x\/}}%
\newcommand{\sgtX}{\mbox{\sgothic X\/}}%
\newcommand{\sgty}{\mbox{\sgothic y\/}}%
\newcommand{\sgtY}{\mbox{\sgothic Y\/}}%
\newcommand{\sgtz}{\mbox{\sgothic z\/}}%
\newcommand{\sgtZ}{\mbox{\sgothic Z\/}}%
%
\newcommand{\Det}{\hbox{\rm det}\mskip2mu}
\newcommand{\cof}{\hbox{\rm cof}\mskip4mu}
\newcommand{\skw}{\hbox{\rm skw}\mskip3mu}
\newcommand{\sym}{\hbox{\rm sym}\mskip3mu}
\newcommand{\Tr}{\hbox{\rm tr}\mskip2mu}
\newcommand{\Rot}{\hbox{\rm Rot}\mskip2mu}
\newcommand{\Lin}{\hbox{\rm Lin}}
\newcommand{\Orth}{\hbox{\rm Orth}}


\newcommand{\zzcirc}{\raisebox{-0.25ex}{$\mskip1mu\circ$}}
\newcommand{\zcirc}[1]{\overset{\zzcirc}{#1}}
\newcommand{\zztri}{\raisebox{-0.25ex}{$\mskip1mu\scriptscriptstyle\triangle$}}
\newcommand{\ztri}[1]{\overset{\zztri}{#1}}
\newcommand{\zzbox}{\raisebox{-0.05ex}{$\mskip1mu\diamond$}}
\newcommand{\zbox}[1]{\overset{\zzbox}{#1}}
%\newcommand{\zztri}{\raisebox{-0.25ex}{$\btri$}}
%\newcommand{\ztri}[1]{\overset{\zztri}{#1}}

%\newcommand{\pards}[2]{\mbox {$\dfrac{\partial #1}{\partial {#2 }}$ }}

\newcommand{\pards}[2]{\mbox{$\dfrac{\partial #1}{\partial {#2 }}$}}

\newcommand{\vs}{\mskip2mu}
\newcommand{\vvs}{\mskip1mu}
%
\newcommand{\trans}{\mskip-2mu\scriptscriptstyle\top} %ELIOT I ADDED THE SPACING%
\newcommand{\sperp}{\scriptscriptstyle\perp\mskip-4mu}
\newcommand{\spar}{\scriptscriptstyle\parallel\mskip-4mu}
\newcommand{\xt}{(\bfx,t)}
\newcommand{\Xt}{(\bfX,t)}
\newcommand{\lj}{[\![}
\newcommand{\rj}{]\!]}
\newcommand{\Blj}{\mbox{$\Big[\kern-0.275em\Big[$}}
\newcommand{\Brj}{\mbox{$\Big]\kern-0.275em\Big]$}}
\newcommand{\zed}{{\bf 0}}
\newcommand{\id}{{\bf 1}}
%
%
\newcommand{\onehalf}{\textstyle{\frac{1}{2}}}
\newcommand{\third}{\textstyle{\frac{1}{3}}}
%
\newcommand{\Grad}{\hbox{\rm grad}\mskip2mu}
\newcommand{\Div}{\hbox{\rm Div}\mskip2mu}                                      %%%%%%
\newcommand{\curl}{\hbox{\rm curl}\mskip2mu}         %%%%%%  DIFFERENTIAL OPERATORS
\newcommand{\Curl}{\hbox{\rm Curl}\mskip2mu}
\newcommand{\divx}{\text{div}\vvs}                   %%%%%%
%
\newcommand{\B}{\text{B}}
\newcommand{\Bt}{\calB_t}                                                                                    %%%%%%
\newcommand{\dBt}{\partial\calB_t}                                                                          %%%%%%  BODY,  PART
%\newcommand{\p}{\text{P}}                                                                                    %%%%%%
\newcommand{\p}{{\calP_\mat}}
\newcommand{\pt}{\calP_t}
\newcommand{\dpt}{\partial\calP_t}
%
\newcommand{\X}{\bfX}
\newcommand{\x}{\bfx}
\newcommand{\y}{\bfchi}
\newcommand{\F}{\bfF}
\newcommand{\U}{\bfU}
\newcommand{\V}{\bfV}
\newcommand{\C}{\bfC}
\newcommand{\R}{\bfR}                                                                                              %%%%%%%
\newcommand{\FT}{\bfF^{\trans}}                                                                         %%%%%%%  BOLDFACE CONTINUUM MECH FIELDS
\newcommand{\Q}{\bfQ}                                                                                        %%%%%%%
\newcommand{\QT}{\bfQ^{\trans}}
\newcommand{\W}{\bfW}
\newcommand{\D}{\bfD}
%\newcommand{\A}{\bfA}
%\newcommand{\S}{\bfS}
%\newcommand{\Se}{\bfS^e}


\newcommand{\tendot}{\mskip-3mu:\mskip-2mu}
\newcommand{\Def}{\overset{\text{def}}{=}}
\newcommand{\n}{\bfn}
\newcommand{\ep}{\varepsilon}%
\newcommand{\thet}{\vartheta}%


%
\newcommand{\scA}{{\scriptscriptstyle\sc A}}%
\newcommand{\scB}{{\scriptscriptstyle\sc B}}%
\newcommand{\scC}{{\scriptscriptstyle\sc C}}%
\newcommand{\scD}{{\scriptscriptstyle\sc D}}%
\newcommand{\scE}{{\scriptscriptstyle\sc E}}%
\newcommand{\scF}{{\scriptscriptstyle\sc F}}%
\newcommand{\scG}{{\scriptscriptstyle\sc G}}%
\newcommand{\scH}{{\scriptscriptstyle\sc H}}%
\newcommand{\scI}{{\scriptscriptstyle\sc I}}%
\newcommand{\scJ}{{\scriptscriptstyle\sc J}}%
\newcommand{\scK}{{\scriptscriptstyle\sc K}}%
\newcommand{\scM}{{\scriptscriptstyle\sc M}}%
\newcommand{\scR}{{\scriptscriptstyle\sc R}}%
\newcommand{\scS}{{\scriptscriptstyle\sc S}}%

\newcommand{\mat}{\text{\tiny R}}%
\newcommand{\spat}{\text{\tiny S}}%
\newcommand{\nspat}{\text{\tiny SS}}%

\newcommand{\ddt}{\frac{\text{d}}{\text{d}t}}
\newcommand{\dt}[1]{\frac{\text{d}#1}{\text{d}t}}
\renewcommand{\v}{\bfv}%
%\renewcommand{\cof}{\scriptscriptstyle\#}
\renewcommand{\cof}{\scriptscriptstyle\sf{C}}
%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%  NEW STUFF
%%%%%%%%%%%%%%%%

\newcommand{\rdot}{\dot{\mskip-3mu\phantom{p}}}


%\newcommand{\zzdot}{\raisebox{-0.25ex}{.}}
%\newcommand{\zdot}[1]{\overset{\zzdot}{#1}}

\newcommand{\RT}{\bfR^{\trans}}

%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%  LALLIT's NEW STUFF
%%%%%%%%%%%%%%%%

%\newcommand{\rdot}{\dot{\mskip-3mu\phantom{p}}}


%\newcommand{\zzdot}{\raisebox{-0.25ex}{.}}
%\newcommand{\zdot}[1]{\overset{\zzdot}{#1}}
%\newcommand{\RT}{\bfR^{\trans}}
\newcommand{\boltz}{\text{\tiny B}}%
\newcommand{\hen}{\text{\tiny H}}%
\newcommand{\calG}{\mathcal{G}}%
\newcommand{\lock}{\text{\tiny L}}%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Ab}{\mbox{\boldmath ${{\bf {\cal A}}}$}}
\newcommand{\Bb}{\mbox{\boldmath ${{\bf {\cal B}}}$}}
\newcommand{\Cb}{\mbox{\boldmath ${{\bf {\cal C}}}$}}
\newcommand{\Db}{\mbox{\boldmath ${{\bf {\cal D}}}$}}
\newcommand{\Eb}{\mbox{\boldmath ${{\bf {\cal E}}}$}}
\newcommand{\Fb}{\mbox{\boldmath ${{\bf {\cal F}}}$}}
\newcommand{\Gb}{\mbox{\boldmath ${{\bf {\cal G}}}$}}
\newcommand{\Hb}{\mbox{\boldmath ${{\bf {\cal H}}}$}}
\newcommand{\Ib}{\mbox{\boldmath ${{\bf {\cal I}}}$}}
\newcommand{\Ibt}{\mbox{\boldmath $\tilde{{\bf {\cal I}}}$}}
\newcommand{\Jb}{\mbox{\boldmath ${{\bf {\cal J}}}$}}
\newcommand{\Kb}{\mbox{\boldmath ${{\bf {\cal K}}}$}}
\newcommand{\Lb}{\mbox{\boldmath ${{\bf {\cal L}}}$}}
\newcommand{\Mb}{\mbox{\boldmath ${{\bf {\cal M}}}$}}
\newcommand{\Nb}{\mbox{\boldmath ${{\bf {\cal N}}}$}}
\newcommand{\Ob}{\mbox{\boldmath ${{\bf {\cal O}}}$}}
\newcommand{\Pb}{\mbox{\boldmath ${{\bf {\cal P}}}$}}
\newcommand{\Qb}{\mbox{\boldmath ${{\bf {\cal Q}}}$}}
\newcommand{\Rb}{\mbox{\boldmath ${{\bf {\cal R}}}$}}
%\newcommand{\Sb}{\mbox{\boldmath ${{\bf {\cal S}}}$}}
\newcommand{\Tb}{\mbox{\boldmath ${{\bf {\cal T}}}$}}
\newcommand{\Ub}{\mbox{\boldmath ${{\bf {\cal U}}}$}}
\newcommand{\Vb}{\mbox{\boldmath ${{\bf {\cal V}}}$}}
\newcommand{\Wb}{\mbox{\boldmath ${{\bf {\cal W}}}$}}
\newcommand{\Xb}{\mbox{\boldmath ${{\bf {\cal X}}}$}}
\newcommand{\Yb}{\mbox{\boldmath ${{\bf {\cal Y}}}$}}
\newcommand{\Zb}{\mbox{\boldmath ${{\bf {\cal Z}}}$}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\calU}{\mathcal{U}}%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\thA}{\mbox{$\Bbb{A}$}}
\newcommand{\thB}{\mbox{$\Bbb{B}$}}
\newcommand{\thC}{\mbox{$\Bbb{C}$}}
\newcommand{\thD}{\mbox{$\Bbb{D}$}}
\newcommand{\thE}{\mbox{$\Bbb{E}$}}
\newcommand{\thF}{\mbox{$\Bbb{F}$}}
\newcommand{\thG}{\mbox{$\Bbb{G}$}}
\newcommand{\thH}{\mbox{$\Bbb{H}$}}
\newcommand{\thI}{\mbox{$\Bbb{I}$}}
\newcommand{\thJ}{\mbox{$\Bbb{J}$}}
\newcommand{\thK}{\mbox{$\Bbb{K}$}}
\newcommand{\thL}{\mbox{$\Bbb{L}$}}
\newcommand{\thM}{\mbox{$\Bbb{M}$}}
\newcommand{\thN}{\mbox{$\Bbb{N}$}}
\newcommand{\thO}{\mbox{$\Bbb{O}$}}
\newcommand{\thP}{\mbox{$\Bbb{P}$}}
\newcommand{\thQ}{\mbox{$\Bbb{Q}$}}
\newcommand{\thR}{\mbox{$\Bbb{R}$}}
\newcommand{\thS}{\mbox{$\Bbb{S}$}}
\newcommand{\thT}{\mbox{$\Bbb{T}$}}
\newcommand{\thU}{\mbox{$\Bbb{U}$}}
\newcommand{\thV}{\mbox{$\Bbb{V}$}}
\newcommand{\thW}{\mbox{$\Bbb{W}$}}
\newcommand{\thX}{\mbox{$\Bbb{X}$}}
\newcommand{\thY}{\mbox{$\Bbb{Y}$}}
\newcommand{\thZ}{\mbox{$\Bbb{Z}$}}

\newcommand{\sdiv}{\hbox{\rm div}\mskip2mu}
\newcommand{\scurl}{\hbox{\rm curl}\mskip2mu}
\newcommand{\grad}{\text{grad}\,}

\newcommand{\pardd}[2]{\mbox{${\dfrac{\partial^2}{\partial {#1} \partial{#2}}}$}}
% \newcommand{\pards}[2]{\mbox { $\dfrac{ \partial #1 }{ \partial {#2 } }$ } }
\newcommand{\pardt}[2]{\mbox{${\dfrac{\partial }{\partial {#2}  } {#1} }$}}
\newcommand{\threedot}{\mskip1mu\raisebox{0.1ex}.\mskip-5mu\raisebox{0.6ex}.\mskip-5mu\raisebox{1.1ex}.\mskip1mu}
\newcommand{\somega}{\boldsymbol{\omega}}%
\newcommand{\kappab}{\boldsymbol{\kappa}}%
\newcommand{\kappabb}{\bar{\boldsymbol{\kappa}}}%
%%
\newcommand{\T}{\bfT}
\newcommand{\Te}{\bfT^e}
\newcommand{\Me}{\bfM^e}
\newcommand{\Tealpha}{\bfT^{e\,(\alpha)}}
\newcommand{\Talpha}{\bfT^{(\alpha)}}
\newcommand{\Tv}{\bfT^v}
\newcommand{\Tp}{\bfT^p}
\newcommand{\Tpk}{\bfT_{\text{2pk}}}
\newcommand{\pk}{\text{\tiny PK}}%
\newcommand{\kk}{\text{\tiny K}}%

\newcommand{\Tmat}{\bfT_{\mat}}
\newcommand{\mvs}{\mskip-2mu}

\newcommand{\h}{\bfh}
\newcommand{\DelX}{\Delta\X}
\newcommand{\Delx}{\Delta\x}
\newcommand{\Delv}{\Delta v}
\newcommand{\DelvR}{\Delta v_{\mat}}
\newcommand{\Dela}{\Delta a}
\newcommand{\DelaR}{\Delta a_{\mat}}
\newcommand{\subt}{_{(t)}}
\newcommand{\pullT}{\bbP}
\newcommand{\pullN}{\underline{\bbP}}
\newcommand{\pullTi}{\bbP^{-1}}
\newcommand{\pullNi}{\underline{\bbP}^{-1}}
\newcommand{\vecpullT}{\bfP}
\newcommand{\vecpullN}{\underline{\bfP}}
\newcommand{\vecpullTi}{\bfP^{-1}}
\newcommand{\vecpullNi}{\underline{\bfP}^{-1}}
\newcommand{\ts}{\bft_{\mskip-2mu\scriptscriptstyle\calS}}
\newcommand{\SR}{\text{S}}
\newcommand{\SO}{\calS}
\newcommand{\SRt}{\SR(t)}
\newcommand{\SOt}{\calS(t)}
\newcommand{\VR}{V_{\mat}}
\newcommand{\mR}{\bfm_{\mat}}
\newcommand{\PR}{\bfP_{\mskip-3mu\mat}}
\newcommand{\doty}{\dot{\y}}
\newcommand{\zp}[1]{{#1}^{\scriptscriptstyle+}}
\newcommand{\zm}[1]{{#1}^{\scriptscriptstyle-}}
\newcommand{\zpm}[1]{{#1}^{\scriptscriptstyle\pm}}
\newcommand{\tR}{\text{R}}
\newcommand{\IB}{\calI_{\bfB}}
\newcommand{\Iid}{\calI_{\bf1}}
\newcommand{\IBt}{\tilde{\calI}_{\bfB}}
\newcommand{\jdR}{\jmath_{\scriptscriptstyle\partial\mskip-2mu R}}
\newcommand{\negzeta}{\scriptscriptstyle\neg\mskip-9.75mu\zeta}
\newcommand{\calY}{\mathcal{Y}}%
\newcommand{\nsites}{n^{\text{sites}}}

\newcommand{\cond}{\text{\small K}}%
\newcommand{\enth}{\text{\small H}}%
\newcommand{\gibb}{\text{\small G}}%
\newcommand{\peq}{ p_{\rm eq} }%


\newcommand{\Sym}{\text{sym}}
\newcommand{\Symz}{\text{sym}_0}
\newcommand{\Fe}{\bfF^e}
%\newcommand{\Fetilde}{\tilde{\bfF}^{e}}
\newcommand{\Fp}{\bfF^p}
\newcommand{\Fei}{\bfF^{e-1}}
\newcommand{\Fet}{\bfF^{e\,\trans}}
\newcommand{\Feit}{\bfF^{e-\trans}}
\newcommand{\Fpi}{\bfF^{p-1}}
\newcommand{\Le}{\bfL^e}
\newcommand{\Lp}{\bfL^p}
\newcommand{\Dp}{\bfD^p}
\newcommand{\Dptilde}{\tilde{\bfD}^{p}}
         %%%%%%%%%%
\newcommand{\Wp}{\bfW^s}           %%%%%%%%%%
\newcommand{\De}{\bfD^e}           %%%%%%%%%%   PLASTICITY MACROS
\newcommand{\We}{\bfW^e}
\newcommand{\Ed}{\bfE^d}
\newcommand{\Ee}{\bfE^e}           %%%%%%%%%%
\newcommand{\Ep}{\bfE^p}
\newcommand{\He}{\bfH^e}           %%%%%%%%%%
\newcommand{\Hp}{\bfH^p}
\newcommand{\dev}{\text{dev}}
\newcommand{\Ce}{\bfC^e}
\newcommand{\Cedot}{\dot{\bfC}^e}
\newcommand{\Eedot}{\dot{\bfE}^e}
\newcommand{\Epdot}{\dot{\bfE}^p}
\newcommand{\Epdoto}{\dot{\bfE}^p_0}
\newcommand{\Np}{\bfN^p}
%
%\newcommand{\Mback}{\bfM^{(\alpha)}_{\text{back}}}
\newcommand{\Mback}{\bfM_{\text{back}}}
%\newcommand{\Meff}{\Mealpha_{\text{eff}}}
\newcommand{\Meff}{\Me_{\text{eff}}}
\newcommand{\Medot}{\dot{\bfM}{}^e}
\newcommand{\prestar}{{}_*\mskip-2mu}
%\newcommand{\epdot}{\dot\ep^p}
%
\newcommand{\epdot}{\dot{\epsilon}^{p} }
%
\newcommand{\ebarp}{\mbox{$\varepsilon^p$}}
\newcommand{\ebarpdot}{\mbox{$\dot{\varepsilon}{}^p$}}
\newcommand{\nup}{\mbox{$\nu^p$}}
\newcommand{\es}{\mbox{$S$}}
\newcommand{\cee}{\mbox{$C$}}
\newcommand{\hh}{\mbox{$h$}}
\newcommand{\Tback}{\mbox{$\bfT_{\text{back}}$}}
\newcommand{\To}{\mbox{$\bfT_0$}}
\newcommand{\taub}{\mbox{$\bar\tau$}}
\newcommand{\pbar}{\mbox{$\bar{p}$}}
\newcommand{\gammab}{\mbox{$\bar\gamma$}}
\newcommand{\etab}{\mbox{$\bar\eta$}}
\newcommand{\matt}{\text{\tiny M}}%
\newcommand{\rel}{\text{\tiny I}}%
%\newcommand{\Trel}{\T^e_{\rel\rel}}
\newcommand{\Trel}{\T_{\rel\rel}}
%\newcommand{\ICe}{\calI_{\Cealpha}}
%\newcommand{\IA}{\calI_{\Aalpha}}
\newcommand{\ICe}{\calI_{\Ce}}
\newcommand{\Cdis}{\C_{\dis} }
\newcommand{\ICdis}{\calI_{\Cdis}}
\newcommand{\ICedis}{\calI_{\Ce_\dis}}
\newcommand{\IA}{\calI_{\A}}
\newcommand{\IBpe}{\calI_{\Bpe}}
\newcommand{\IC}{\calI_{\C}}
\newcommand{\Ue}{\bfU^e}
\newcommand{\Ve}{\bfV^e}
\newcommand{\Up}{\bfU^p}
\newcommand{\Vp}{\bfV^p}
\newcommand{\Rp}{\bfR^p}
\newcommand{\Be}{\bfB^e}
\newcommand{\Bp}{\bfB^p}
\newcommand{\Yp}{\bfY^p}
%
%\newcommand{\Ce}{\bfC^e}
\newcommand{\Cp}{\bfC^p}
\newcommand{\rot}{\text{Orth}^+}
\newcommand{\ski}{\mbox{\boldmath$\xi$}}
\newcommand{\Imeff}{\calI_{\Meff}}
%\newpage


\newcommand{\Fealpha}{\bfF^{e\,(\alpha)}}
\newcommand{\Fealphat}{\tilde{\bfF}^{e\,(\alpha)}}
\newcommand{\Fedotalpha}{\dot{\bfF}^{e\,(\alpha)}}
\newcommand{\Fedot}{\dot{\bfF}^{e}}
\newcommand{\Realpha}{\bfR^{e\,(\alpha)}}
\newcommand{\Uealpha}{\bfU^{e\,(\alpha)}}
\newcommand{\Vealpha}{\bfV^{e\,(\alpha)}}
\newcommand{\Aalpha}{\bfA^{(\alpha)}}
\newcommand{\Bealpha}{\bfB^{e\,(\alpha)}}
\newcommand{\Cealpha}{\bfC^{e\,(\alpha)}}
\newcommand{\Cedotalpha}{\dot{\bfC}^{e\,(\alpha)}}
\newcommand{\Fpalpha}{\bfF^{p\,(\alpha)}}
\newcommand{\Lpalpha}{\bfL^{p\,(\alpha)}}
\newcommand{\Mpalpha}{\bfM^{p\,(\alpha)}}
\newcommand{\Dpalphat}{\tilde{\bfD}^{p\,(\alpha)}}
\newcommand{\Dpalpha}{\bfD^{p\,(\alpha)}}
\newcommand{\Dpalphab}{\bar{\bfD}^{p\,(\alpha)}}
\newcommand{\Npalpha}{\bfN^{p\,(\alpha)}}
\newcommand{\lpalpha}{l^{p\,(\alpha)}}
\newcommand{\dpalpha}{d^{p\,(\alpha)}}
\newcommand{\deep}{d^{p}}
\newcommand{\Npalphab}{\bar{\bfN}^{p\,(\alpha)}}
\newcommand{\nupalpha}{d^{p\,(\alpha)}}
\newcommand{\nupalphab}{\bar{d}^{p\,(\alpha)}}
\newcommand{\Wpalpha}{\bfW^{p\,(\alpha)}}
\newcommand{\Upalpha}{\bfU^{p\,(\alpha)}}
\newcommand{\Cpalpha}{\bfC^{p\,(\alpha)}}
\newcommand{\Vpalpha}{\bfV^{p\,(\alpha)}}
\newcommand{\Bpalpha}{\bfB^{p\,(\alpha)}}
\newcommand{\Rpalpha}{\bfR^{p\,(\alpha)}}
\newcommand{\Ypalpha}{\bfY^{p\,(\alpha)}}
\newcommand{\Lealpha}{\bfL^{e\,(\alpha)}}
\newcommand{\Dealpha}{\bfD^{e\,(\alpha)}}
\newcommand{\Eealpha}{\bfE^{e\,(\alpha)}}
\newcommand{\Wealpha}{\bfW^{e\,(\alpha)}}
\newcommand{\Qalpha}{\bfQ^{(\alpha)}}
\newcommand{\Qalphat}{\bfQ^{(\alpha)\,\trans}}
\newcommand{\Lealphat}{\tilde{\bfL}^{e\,(\alpha)}}
\newcommand{\Salpha}{S^{(\alpha)}}
\newcommand{\skialpha}{\bfxi^{(\alpha)}}
\newcommand{\xialpha}{\xi^{(\alpha)}}
\newcommand{\halpha}{h^{(\alpha)}}
\newcommand{\ealpha}{\psi^{(\alpha)}}
\newcommand{\lalpha}{\mbox{$\bar{\lambda}^{e\,(\alpha)} $}}
\newcommand{\Pealpha}{\bfP^{e\,(\alpha)}}
\newcommand{\Pe}{\bfP^e}
\newcommand{\Sealpha}{\bfS^{e\,(\alpha)}}
\newcommand{\Mealpha}{\bfM^{e\,(\alpha)}}
 \newcommand{\Jealpha}{J^{e\,(\alpha)}}
\newcommand{\Yalpha}{Y^{(\alpha)}}
\newcommand{\npalpha}{\nu^{p\,(\alpha)}}
\newcommand{\Sigmae}{\boldsymbol{\Sigma}^{e\,(\alpha)}}
%
\newcommand{\bfSigmae}{\boldsymbol{\Sigma}^{e}}
%
\newcommand{\Sigmaeo}{\boldsymbol{\Sigma}^{e}_0}
%
\newcommand{\Sigmaealpha}{\boldsymbol{\Sigma}^{e\,(\alpha)}}
%
\newcommand{\Sigmaealphao}{\boldsymbol{\Sigma}^{e\,(\alpha)}_0}
\newcommand{\Mealphao}{\bfM^{e\,(\alpha)}_0}
%\newcommand{\bfxi}{\boldsymbol{\xi}}%
\newcommand{\taup}{\bar{\tau}_p}
\newcommand{\prt}{\text{P}}
\newcommand{\symz}{\text{sym}_0}
%\newcommand{\rot}{\text{Orth}^+}
%\newcommand{\es}{S}
\newcommand{\tauact}{ \tau_{\text{e}}}
\newcommand{\dis}{\text{dis}}
\newcommand{\vol}{\text{vol}}
\newcommand{\maxm}{\text{max}}
\newcommand{\refn}{\text{ref}}
\newcommand{\dee}{\mbox{$d$}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\dX}{\bfd\bfX}
%\newcommand{\dx}{\bfd\bfx}
\newcommand{\lX}{\bfu_{\text{R}}}
\newcommand{\lx}{\bar{\bfu}}
\newcommand{\MX}{\calM_{\bfX}}
\newcommand{\refX}{\text{Ref}_{\bfX}}
\newcommand{\defx}{\text{Def}_{\bfx}}
\newcommand{\nX}{\bfn_{\text{R}}}
\newcommand{\nx}{\bar{\bfn}}
\newcommand{\Tpalpha}{\bfT^{p\,(\alpha)}}
\newcommand{\palpha}{\psi^{(\alpha)}}
%
%\newcommand{\S}{\bfS}
\newcommand{\Se}{\bfS^e}
%\newcommand{\Sealpha}{\bfS^{e\,(\alpha)}}
%\newcommand{\Fedotalpha}{\dot\bfF^{e\,(\alpha)}}
\newcommand{\Sv}{\bfS^v}
\newcommand{\Sp}{\bfS^p}
\newcommand{\Spalpha}{\bfS^{p\,(\alpha)}}
\newcommand{\eSalpha}{S^{(\alpha)}}
%
\newcommand{\Tpdis}{\hat{\bfT}^p_{\text{dis}}}
\newcommand{\Tpen}{\hat{\bfT}^p_{\text{en}}}
\newcommand{\TX}{\bfT(\bfX)}

\newcommand{\lamp}{\bar\lambda^p}
\newcommand{\sign}{\text{sign}}
\newcommand{\en}{\text{en}}
\newcommand{\diss}{\text{diss}}
\newcommand{\Fpe}{\Fp_\en}
\newcommand{\Upe}{\Up_\en}
\newcommand{\Vpe}{\Vp_\en}
\newcommand{\Rpe}{\bfR^p_\en}
\newcommand{\Fpd}{\Fp_\dis}
\newcommand{\Upd}{\Up_\dis}
\newcommand{\Vpd}{\Vp_\dis}
\newcommand{\Rpd}{\bfR^p_\dis}
\newcommand{\Epe}{\bfE^p_\en}

%
\newcommand{\Cpe}{\Cp_\en}
\newcommand{\Bpe}{\Bp_\en}
\newcommand{\Bpedot}{\dot\bfB^p_\en}
\newcommand{\Cpedot}{\dot\bfC^p_\en}
%
\newcommand{\Cpd}{\Cp_\dis}
\newcommand{\Bpd}{\Bp_\dis}
%
\newcommand{\Lpe}{\Lp_\en}
\newcommand{\Lpd}{\Lp_\dis}
\newcommand{\Dpe}{\Dp_\en}
\newcommand{\Dpd}{\Dp_\dis}
\newcommand{\Dpetilde}{\tilde\bfD^p_\en}
\newcommand{\Dpdtilde}{\tilde\bfD^p_\dis}
%
\newcommand{\Wpe}{\Wp_\en}
\newcommand{\Wpd}{\Wp_\dis}
%
\newcommand{\Tpe}{\Tp_\en}
\newcommand{\Tpd}{\T_\dis}
\newcommand{\Td}{\T_\dis}
\newcommand{\Spe}{\bfS_\en}
\newcommand{\Spd}{\bfS_\dis}
\newcommand{\Men}{\bfM^\en}
\newcommand{\Mpd}{\bfM_\dis}
\newcommand{\Mpe}{\bfM^p_\en}

\newcommand{\Fpedot}{\dot{\bfF}^{p}_\en}
\newcommand{\Fpetilde}{\tilde{\bfF}^{p}_\en}
\newcommand{\Letilde}{\tilde\bfL^e}
\newcommand{\bfvtilde}{\tilde\bfv}


\newcommand{\ft}{\mbox{${\bf F}$}}
\newcommand{\fte}{\mbox{${\bf F}^e$}}
\newcommand{\ftstar}{\mbox{${\bf F}^e$}}
\newcommand{\ftetr}{\mbox{${\bf F}^e_*$}}
\newcommand{\ftp}{\mbox{${\bf F}^{p}$}}
\newcommand{\ftpb}{\mbox{$\bar{\bf F}^p$}}
\newcommand{\ue}{\mbox{${{\bf U}^e}$}}
\newcommand{\uetr}{\mbox{${{\bf U}^e_*}$}}
\newcommand{\ve}{\mbox{${{\bf V}^e}$}}
\newcommand{\ce}{\mbox{${{\bf C}^e}$}}
\newcommand{\re}{\mbox{${{\bf R}^e}$}}
\newcommand{\retr}{\mbox{${{\bf R}^e_*}$}}
\newcommand{\ee}{\mbox{${{\bf E}^e}$}}
\newcommand{\estar}{\mbox{${{\bf E}^e}$}}
\newcommand{\ebe}{\mbox{${\bar{\bf E}^e}$}}
\newcommand{\ebiottr}{\mbox{${{\bf E}^B_*}$}}
\newcommand{\ebst}{\mbox{${{\bf E}^B_t}$}}
\newcommand{\ebetr}{\mbox{${\bar{\bf E}^e_*}$}}
%
\newcommand{\lte}{\mbox{${\bf L}^e$}}
\newcommand{\ltp}{\mbox{${\bf L}^{p}$}}
\newcommand{\dte}{\mbox{${\bf D}^e$}}
\newcommand{\dtp}{\mbox{${\bf D}^p$}}
\newcommand{\epstdp}{\mbox{$\dot{\tilde{\epsilon}}^p$}}
\newcommand{\ede}{\mbox{$\dot{\epsilon}_e$}}
\newcommand{\edo}{\mbox{$\dot{\epsilon}_o$}}
\newcommand{\edm}{\mbox{$\dot{\epsilon}_m$}}
\newcommand{\edpm}{\mbox{$\dot{\epsilon}^p_m$}}
\newcommand{\wte}{\mbox{${\bf W}^e$}}
\newcommand{\wtp}{\mbox{${\bf W}^p$}}
\newcommand{\wtwp}{\mbox{${\bf W}^{\mbox{wp}}$}}
%
\newcommand{\ltb}{\mbox{$\bar{\bf L}$}}
\newcommand{\dtb}{\mbox{$\bar{\bf D}$}}
\newcommand{\wtb}{\mbox{$\bar{\bf W}$}}
\newcommand{\ltpb}{\mbox{$\bar{{\bf L}}^p$}}
\newcommand{\dtpb}{\mbox{$\bar{{\bf D}}^p$}}
\newcommand{\wtpb}{\mbox{$\bar{{\bf W}}^p$}}
\newcommand{\stress}{\mbox{${\bf T}$}}
\newcommand{\rb}{\mbox{${{\bf r}}$}}
%\newcommand{\prt}{\text{P}}
\newcommand{\tildeT}{\mbox{$\tilde{\bf T}$}}
%\newcommand{\sign}{\text{sign}\,}
\newcommand{\npone}{\text{n+1}\,}
\newcommand{\epsbp}{\mbox{$\bar{{\epsilon}}^p $}}
\newcommand{\trial}{\text{trial}\,}
%

\newcommand{\Meffd}{\mbox{$(\bfM^{e}_{\text{eff}})_0$}}
\newcommand{\xidot}{\mbox{$\dot{\xi}$}}
\newcommand{\gammabp}{\mbox{$\bar{{\gamma}}^p $}}

\newcommand{\tildevel}{\mbox{$\tilde{\dot\y}$}}
\newcommand{\Fetilde}{\mbox{$\tilde{\Dot{\bfF}}{}^e$}}


%%%%%%%%%%%%%%%%%%%%%%%%%% SWELLING MACROS

%\newcommand{\Fm}{\bfF^m}
%%\newcommand{\Fmtilde}{\tilde{\bfF}^{e}}
\newcommand{\Fs}{\bfF^s}
%\newcommand{\Fmi}{\bfF^{m-1}}
%\newcommand{\Fmt}{\bfF^{m\,\trans}}
%\newcommand{\Fmit}{\bfF^{m-\trans}}
%\newcommand{\Fsi}{\bfF^{s-1}}
%\newcommand{\Lm}{\bfL^m}
%\newcommand{\Ls}{\bfL^s}
%\newcommand{\Ds}{\bfD^s}
%\newcommand{\Dstilde}{\tilde{\bfD}^{s}}
%         %%%%%%%%%%
%\newcommand{\Ws}{\bfW^s}           %%%%%%%%%%
%\newcommand{\Dm}{\bfD^m}           %%%%%%%%%%
%\newcommand{\Wm}{\bfW^m}
%\newcommand{\Ed}{\bfE^d}
%%\newcommand{\Ee}{\bfE^e}           %%%%%%%%%%
%%\newcommand{\Ep}{\bfE^p}
%%\newcommand{\He}{\bfH^e}           %%%%%%%%%%
%%\newcommand{\Hp}{\bfH^p}
%%\newcommand{\dev}{\text{dev}}
%%\newcommand{\Ce}{\bfC^e}
%%\newcommand{\Cedot}{\dot{\bfC}^e}
%%\newcommand{\Eedot}{\dot{\bfE}^e}
%%\newcommand{\Epdot}{\dot{\bfE}^p}
%%\newcommand{\Epdoto}{\dot{\bfE}^p_0}
%%\newcommand{\Np}{\bfN^p}

\newcommand{\pol}{\text{\tiny pol}}%
\newcommand{\sol}{\text{\tiny sol}}%
\newcommand{\eff}{\text{\tiny eff}}
\newcommand{\Gee}{\mbox{$G$}}
\newcommand{\Kay}{\mbox{$K$}}
\newcommand{\cmat}{c_{\mat}}
\newcommand{\ucmat}{\upsilon c_{\mat}}
\newcommand{\ocmat}{\Omega c_{\mat}}
\newcommand{\Pee}{P}
\newcommand{\extra}{\text{\tiny act}}
\newcommand{\mix}{\text{\tiny mix}}


